Chainer: A Deep Learning Framework for Accelerating the Research Cycle

Software frameworks for neural networks play a key role in the development and application of deep learning methods. In this paper, we introduce the Chainer framework, which intends to provide a flexible, intuitive, and high performance means of implementing the full range of deep learning models needed by researchers and practitioners. Chainer provides acceleration using Graphics Processing Units with a familiar NumPy-like API through CuPy, supports general and dynamic models in Python through Define-by-Run, and also provides add-on packages for state-of-the-art computer vision models as well as distributed training.

==> advanced.tex <==
\section{Advanced Features}
\todo[inline]{Write: Trainer, ChainerMN/CV/RL/UI(/Chemistry?)}







==> implementation.tex <==
\section{Implementation}
\todo[inline]{Python-based implementation, GPU implementation backed by CuPy, iDeep backend, computational graph implementation detail?}

